Zero-Shot AutoML with Pretrained Models

Given a new dataset D and a low compute budget, how should we choose a pre-trained model to fine-tune to D, and set the fine-tuning hyperparameters without risking overfitting, particularly if D is small? Here, we extend automated machine learning (AutoML) to best make these choices. Our domain-independent meta-learning approach learns a zero-shot surrogate model which, at test time, allows to select the right deep learning (DL) pipeline (including the pre-trained model and fine-tuning hyperparameters) for a new dataset D given only trivial meta-features describing D such as image resolution or the number of classes. To train this zero-shot model, we collect performance data for many DL pipelines on a large collection of datasets and meta-train on this data to minimize a pairwise ranking objective. We evaluate our approach under the strict time limit of the vision track of the ChaLearn AutoDL challenge benchmark, clearly outperforming all challenge contenders.

==> 6_discussion.tex <==
\section{Discussion}


\label{sec:ack}

==> alg/algALC.tex <==
\begin{algorithm}[p]
\caption{Area Under the Learning Curve}
\label{alg:alc}
\begin{algorithmic}
    % \ttfamily
    \STATE \textbf{Input:} AUC $\gets$ Area Under ROC Curve
    \STATE $T \gets 1200$
    \STATE $t_0 \gets 60$
    \STATE Get test set $\vec{p}_i$ on time $t_i$ of $m$ time steps where $i \in \{0, \ldots, m-1\}$
    \FORALL{$\vec{p}_i$}
        \STATE $s_i \gets 2*AUC(\vec{p}_i)-1$ 
    \ENDFOR
    \STATE $s(t) \gets step\_fn(\vec{s})$ 
    \STATE $ALC = \frac{1}{\log{(1+T/t_0)}} \int_{0}^{T} \frac{s(t)}{t+t_0} dt$
\end{algorithmic}
\end{algorithm}

==> autodl-comp-details.tex <==

\paragraph{Deatils about the AutoDL Competition} 
% TODO @Ekrem
% winning solutions
ChaLearn’s AutoDL Challenge~\cite{Liu2021_Autodl} has a unique setting with its rules and evaluation metric that lays stress on anytime performance. It is a follow-up, united competition, of previous competitions took place on five (image, video, speech, text, tabular) main domains. Furthermore, the qualifying baseline is the winner solutions of AutoCV/CV2, AutoSpeech, AutoNLP, AutoWSL~\cite{liu_autodl_2019} which is a very strong baseline to overcome and requires competitors to be very versatile. 

The image track baseline, the AutoCV/CV2 winner \citealt{Baek2020_Autoclint}, propose a lighter version of Fast AutoAugment~\cite{Lim2019_FastAutoAugment}, which was already approximately 1000 times faster than AutoAugment~\cite{Cubuk2019_AutoAugment}, suitable under tight budgets. They further improve initializing ImageNet~\cite{krizhevsky_imagenet_2012} pretrained ResNet-18~\cite{he-corr15a} as their base architecture and also introduce few novel hyperparameters (with their hard-coded values), extends the model's control during the AutoDL training/evaluation procedure. 

On the AutoDL Challenge, all the winning solutions use the AutoCV winner code above as a skeleton and build their methods on top. They introduce modifications, such as, switching to more stable architectures like ResNet-9 at some point in training (DeepWisdom), ensembling latest $n$ predictions (DeepBlueAI) and data adaptive preprocessing (PASA NJU). 

In despite to the abundance of meta-learning methods and applications, the number of evaluation alternatives are scarce. ~\citealt{Zhai2019_VTAB} tries to resolve the issue by introducing a set of 19 vision tasks each including number of labelled samples with low sample complexity and evaluating several representation learning algorithms on this benchmark. ~\citealt{triantafillou_meta-dataset:_2019} also introduced a meta-dataset of few-shot image classification tasks and benchmarked several prominent meta-learning baselines. A more recent work ~\citealt{Dumoulin2021_VTAB_MD} combines the two benchmarks and compares Big Transfer(BiT)~\cite{Kolesnikov2020_Bit} against aforementioned baselines.
%} by creating a handful set of few-shot classification datasets. 

==> fig/barChartAutoDL.tex <==
\begin{figure}[ht]
\begin{centering}

    {\includegraphics[scale=0.35]{fig/images/pairwise_performance_bar_chart_Simple.png}}

    {\includegraphics[scale=0.35]{fig/images/significant_pairwise_performance_bar_chart_Simple.png}}

    {\includegraphics[scale=0.35]{fig/images/pairwise_performance_bar_chart_Simple (tuned).png}}

    {\includegraphics[scale=0.35]{fig/images/significant_pairwise_performance_bar_chart_Simple (tuned).png}}
    
    \caption[]{\textbf{Pairwise performances of solutions} These plots compare our solutions with the winner (including \textit{automl\_freiburg} since they have achieved on par score with the first place on AutoCV track) solutions. On charts \textbf{a} and \textbf{c}, we compare the solutions by their mean performances and put a notch in better solution's belt. On charts \textbf{b} and \textbf{d}, we only count if a solution performs significantly better (performances are one standard deviation apart) on a task.}
    \label{fig:barchart_autodl}
\end{centering}
\end{figure}

==> fig/boxPlotALL.tex <==
\begin{figure}[ht!]
\begin{centering}

    \subfigure[]{\includegraphics[scale=0.22]{fig/images/benchmarking_boxplot/all.png}}
    \subfigure[]{\includegraphics[scale=0.22]{fig/images/benchmarking_boxplot/all_nauc.png}}
    \subfigure[]{\includegraphics[scale=0.22]{fig/images/benchmarking_boxplot/all_acc.png}}
    
    \caption[]{\textbf{Benchmarking of all solutions} over 525 datasets and 10 repetitions.}
    \label{fig:benchmark_boxplot_all}
\end{centering}
\end{figure}

==> fig/boxPlotMF.tex <==
\begin{figure}[ht]
\begin{centering}

    {\includegraphics[scale=0.3]{fig/images/benchmarking_boxplot/mf.png}}

    \caption[]{\textbf{Ablation of our method with or without (NO-MF) meta-features} over 525 datasets and 10 repetitions. } % Ablation score matches with the single-best, showing that performance ceiling of having no meta-features is the same as of having no dataset adaptation.
    \label{fig:benchmark_boxplot_mf}
\end{centering}
\end{figure}

==> tab/tabALCrankingMF.tex <==
\begin{table}[ht]
    \caption[Table caption]{\textbf{Ranking meta-feature devoid surrogate against winner solutions}}
    \begin{center}
    \begin{tabular}{l c}
        \hline
        \textbf{Solution} & \textbf{Rank (ALC)}\\
        \hline
        DeepWisdom & $2.51\pm0.04$ \\%& $2.92$ & $2.40$\\
        DeepBlueAI & $2.65\pm0.02$ \\%& $2.73$ & $2.62$\\
        PASA NJU & $3.04\pm0.04$ \\%& $2.41$ & $\mathbf{2.3}$\\
        ZAP-HPO NO-MF & $\mathbf{1.80\pm0.02}$ \\%& $\mathbf{1.95}$ & $2.68$\\
        \hline
    \end{tabular}
    \end{center}
    \label{tab:ranking_no_mf}
\end{table}

==> tab/tabConfigSpace.tex <==
\begin{table}
    \caption[Table caption]{\textbf{The search space of hyperparameter optimization on AutoDL context} The parameters are grouped according to their "functioning". \textbf{First} category determines the strategies during the 20 minutes of training such as how to validate, when to test etc. These are important decisions in the context of AutoDL challenge that can effect the final ALC. The \textbf{second} category contains generic neural network hyperparameters withal the choice of network architecture. We load and use the architectures with ImageNet pretrained parameters and the \textbf{third} group determines mainly the fine-tuning strategy. Finally, since the neural networks are slow to train and first few seconds are very precious, we use the \textbf{fourth} category to whether to use a simpler model at the beginning of the training.}
\begin{center}
    \begin{tabular}{|l|l|l|}
        \hline
        Name & Type & Value \\ 
        \hline
        CV valid ratio      & \textit{float} & $[0.05, 0.2]$ \\
        Max valid count     & \textit{integer} & $[128, 512]$ \textbf{log} \\
        Max size            & \textit{integer} & $[5, 7]$ \\
        Train info sample   & \textit{integer} & $[128, 512]$ \textbf{log} \\
        Steps per epoch     & \textit{integer} & $[5, 250]$ \textbf{log} \\
        Early epoch         & \textit{integer}& $[1, 3]$ \\
        Skip valid score threshold & \textit{float} & $[0.7, 0.95]$ \\
        Test after at least seconds & \textit{integer} & $[1, 3]$ \\
        Test after at least seconds max & \textit{integer} & $[60, 120]$ \\
        Test after at least seconds step & \textit{integer} & $[2, 10]$ \\
        Max inner loop ratio & \textit{float} & $[0.1, 0.3]$ \\
        \hline
        Batch size & \textit{integer} & $[16, 64]$ \textbf{log} \\
        Learning rate & \textit{float} & $[10^{-5}, 10^{-1}]$ \textbf{log} \\
        Min learning rate & \textit{float} & $[10^{-8}, 10^{-5}]$ \textbf{log} \\
        Weight decay & \textit{float} & $[10^{-5}, 10^{-2}]$ \textbf{log} \\
        Momentum & \textit{float} & $[0.01, 0.99]$ \\
        Optimizer & \textit{categorical} & \{SGD, Adam, AdamW\} \\
        Nesterov & \textit{categorical} & \{true, false\} \\
        Amsgrad & \textit{categorical} & \{true, false\} \\
        Scheduler & \textit{categorical} & \{plateau, cosine\} \\
        Architecture & \textit{categorical} & \{ResNet18, EffNet-b0, EffNet-b1, EffNet-b2\} \\
        \hline
        Freeze portion & \textit{categorical} & \{$0.0$, $0.1$, $0.2$, $0.3$, $0.4$, $0.5$\}\\
        Warm-up multiplier & \textit{categorical} & \{$1.0$, $1.5$, $2.0$, $2.5$, $3.0$\}\\
        Warm-up epoch & \textit{integer} & $[3, 6]$ \\
        \hline
        First simple model & \textit{categorical} & \{true, false\} \\
        Simple model & \textit{categorical} & \{SVC, NuSVC, RF, LR\} \\
        \hline
    \end{tabular}
    \end{center}
    \label{tab:ss_autodl}
\end{table}
